Adaptation Across Extreme Variations using Unlabeled Domain Bridges

We tackle an unsupervised domain adaptation problem for which the domain discrepancy between labeled source and unlabeled target domains is large, due to many factors of inter and intra-domain variation. While deep domain adaptation methods have been realized by reducing the domain discrepancy, these are difficult to apply when domains are significantly unalike. In this work, we propose to decompose domain discrepancy into multiple but smaller, and thus easier to minimize, discrepancies by introducing unlabeled bridging domains that connect the source and target domains. We realize our proposal through an extension of the domain adversarial neural network with multiple discriminators, each of which accounts for reducing discrepancies between unlabeled (bridge, target) domains and a mix of all precedent domains including source. We validate the effectiveness of our method on several adaptation tasks including object recognition and semantic segmentation.

==> algorithm.tex <==
\begin{algorithm}[t]
\caption{Model training procedure.}
\label{alg:multiple_bridging_domains}
\begin{algorithmic}[1]
\small{
\State {\bfseries Input:} source domain data $X_0$ with label $Y$, bridging domain data $X_m, m\,{=}\,1,...,M$, and target domain data $X_{M+1}$, batch size $n$, and maximum iteration $L$.

\For{$\text{itr} = 1, \ldots, L$}
    \State Sample a batch of source data $\{(x_i^{(0)}, y_i)\}_{i=1}^{n}$, 
    \State bridging data $\{x_i^{(m)}\}_{i=1}^{n}, m\,{=}\,1,...,M$, 
    \State and target data $\{x_i^{(M+1)}\}_{i=1}^{n}$;
    
    \State Extract feature $f(x_i^{(j)})$ for all domains;
    
    \State Update discriminator $d_m(\,\cdot\,;\theta_{d_m})$ by maximizing \eqref{eq:d_m};
    %{\small $$\hat{\mathcal{L}}_{d_m} = \sum_{j=0}^{m-1} \sum_{i=1}^n\log d_m(F^{(j)}_i) + \sum_{i=1}^n\log [1-d_m(F^{(m)}_i)]$$}
    
    \State Update classifier $C(\,\cdot\,;\theta_C)$ by minimizing \eqref{eq:multiple_bridging_obj};
    %{\small $$\hat{\mathcal{L}}_C = -\sum_{i=1}^n y_i\log C(F_i^{(0)})$$}
    
    \State Update feature extractor $f(\,\cdot\,;\theta_f)$ by minimizing \eqref{eq:multiple_bridging_obj}; 
    
    %{\small $$\hat{\mathcal{L}}_C - \sum_{m=1}^{M+1}\hat{\mathcal{L}}_{d_m}$$}
\EndFor
}
\end{algorithmic}
\end{algorithm}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
